Understanding Opinions Towards Climate Change on Social Media

Social media platforms such as Twitter (now known as X) have revolutionized how the public engage with important societal and political topics. Recently, climate change discussions on social media became a catalyst for political polarization and the spreading of misinformation. In this work, we aim to understand how real world events influence the opinions of individuals towards climate change related topics on social media. To this end, we extracted and analyzed a dataset of 13.6 millions tweets sent by 3.6 million users from 2006 to 2019. Then, we construct a temporal graph from the user-user mentions network and utilize the Louvain community detection algorithm to analyze the changes in community structure around Conference of the Parties on Climate Change~(COP) events. Next, we also apply tools from the Natural Language Processing literature to perform sentiment analysis and topic modeling on the tweets. Our work acts as a first step towards understanding the evolution of pro-climate change communities around COP events. Answering these questions helps us understand how to raise people's awareness towards climate change thus hopefully calling on more individuals to join the collaborative effort in slowing down climate change.

==> 040Experiments.tex <==
\section{Experiments}
\subsection{Dataset}
We leverage a historical dataset of 13.6 million climate change tweets sent by 3.6 million users between 2006 and 2019 \cite{effrosynidis2022climate}. In addition to the provided metadata, we retrieve the full text for each tweet. Details about this data collection process can be found in Appendix \ref{sec:data}.

\subsection{Community Detection}
As a first attempt, we hypothesize that the community structure, particularly the number of communities might vary significantly surround climate change events such as COP. Figure~\ref{Fig:adv_stats} shows the evolution of the graph density over time as well as the number of communities detected by the Louvain algorithm as described in Section~\ref{sub:louvain}. Note that the density of the graph also affects the community structure as dense graphs are likely to have smaller number of communities. Outside of the peak at the beginning of the dataset and the peak around COP 17, the graph remains quite dense. On the other hand, the number of communities seem to increase over time with local peaks periodically. 

Next, we examine the community structure of graph snapshots surround COP events (10 weeks before and 10 weeks after) with the Louvain algorithm. Figure~\ref{Fig:cop20and21} shows the change in number of communities around COP 18 to 21. For COP 18 and 19, there is a decrease in the number of communities. For COP 20 and COP 21, there seem to be an increase of communities. Therefore, it is difficult to directly draw conclusion from these observations. This is also expected as the Louvain algorithm is computed based the graph structure alone and doesn't utilize the tweet text and other edge features. 



\subsection{Sentiment Analysis}
From the results that we get from the sentiment of the tweets, we understand that its vague to identify the texts as towards climate change or not. Hence, we consider to not move forward with the sentiments analysis of the tweets as the result seems quiet ambiguous.
By combining sentiment analysis with other techniques such as network analysis and topic modeling, we may gain a deeper understanding of the dynamics of climate change communities on social media and how real-world events shape public opinion. This information can be used to develop effective communication strategies, address misinformation campaigns and promote climate change awareness.

\begin{wrapfigure}{r}{0.4\textwidth} % 'r' indicates right alignment
  \centering
  \includegraphics[width=0.4\textwidth]{figs/sentiment_analysis.png}
  \caption{Distribution of \emph{positive}, \emph{negative} and \emph{neutral} tweets.}
  \label{fig:sentiment_image}
\end{wrapfigure}

\subsection{Topic Modeling}
We first tokenized the tweets data and then trained the mini-batch NMF model on the preprocessed corpus by setting the number of topics as 10. We utilized the scikit-learn toolkit to run mini-batch NMF model. The training algorithm was run for iterations until convergence, i.e., a set of stable topics was obtained.  After the matrix factorization had been done, we looked at the topic-word score matrix $W$ and described each topic by the words with the highest relevance score. 
Figure~\ref{Fig:topics} shows three obtained representative topics with their top 20 words about \emph{politics}, \emph{\ch{CO2} emission}, and \emph{weather}. The \emph{politics} topic is related to politicians (e.g., Trump), organizations (e.g., EPA) and actions to address and mitigate climate change. The \emph{\ch{CO2} emission} topic includes global warming, Arctic ice melting, and sea level rising as consequences of \ch{CO2} emission. The \emph{weather} topic shows people's concern about extreme and abnormal weather caused by global warming. 


==> 050Existing_vs_ML.tex <==
\section{Method benefits}

When comparing our method to existing approaches, one can expect the following benefits:
\begin{itemize}[leftmargin=1pt]
    \item Understanding of both network and NLP context surrounding climate change topics on social media.
    \item One of the first method to examine how climate change related events would affect the discourse on social media.
\end{itemize}

==> 060_NextSteps.tex <==
\section{Next Steps}
For next steps in this project, we are planning to add additional experiments in the following directions. 


\paragraph{Community Detection} First we would like to examine if the detected communities align with opinions on climate change by randomly sampling users from large communities and checking their past tweets and stand on climate change. Next, we would like to implement additional community detection methods to check if the number of communities as well as community assignments are similar to the Louvain algorithm. Lastly, we would like to propose new ways to incorporate text information into community detection methods for the purpose of mining opinion communities on social media. 

Secondly, we would also like to  consider the user-hashtag network. This is a bipartite graph where both users and hashtags are nodes and edges are formed between a user and a hashtag when a user includes a hashtag in their tweet. This network tracks the evolution of climate change related hashtags used in tweets over time as well as how users utilizes different hashtags. We believe that examining how the use of hashtags change around COP events would also be beneficial in understanding opinion dynamics. 

\paragraph{Sentiment Analysis} 
\cite{bert_doi:10.48550/arXiv.1810.04805} BERT, or Bidirectional Encoder Representations from Transformers, is a type of language model developed by Google that has revolutionized the field of natural language processing (NLP). It uses a deep neural network to understand the context of words in a sentence, allowing it to generate highly accurate predictions for the next word in a sequence. BERT is trained on a massive amount of text data, which enables it to capture the nuances of natural language.

BERT and other large language models (LLMs) can be used to analyze tweets related to climate change. By using these models, we can better understand the sentiment of tweets and the attitudes of social media users towards climate change. This can help to identify patterns in social media discourse and detect the spread of misinformation campaigns.

\cite{llm_doi:2303.07205} LLMs have been shown to be highly effective in analyzing social media data, with studies indicating that these models can accurately predict the sentiment of tweets with an accuracy of up to 87\%. By utilizing LLMs, we can analyze large amounts of social media data in a highly efficient manner, allowing us to gain insights into the opinions and attitudes of the public towards climate change.

\paragraph{Incorporating topic modeling and graph learning} When working on a graph, there are two possible sources of information that can be used --- the network structure and the node features. \cite{yang2013community} proposed a community detection method that harnesses node attributes (features) to benefit community detection. As topic modeling is able to learn a topic membership vector for a tweet or a collection of one's tweets, we will use the vector as the node feature and investigate how topic features will influence community detection on the Twitter users in our dataset.  


==> 070General_Considerations.tex <==

 Our analysis provides valuable insights into climate-change-related opinions on Twitter, but it is important to approach social media data analysis with awareness of the ethical considerations and data quality limitations. By being mindful of these factors, future studies can build on our work and contribute to a more comprehensive understanding of public opinion on climate change.

==> Machine_Learning_Methods.tex <==
\section{Methodology}

\subsection{Community Detection on Graphs} \label{sub:louvain}
Community detection is one of the fundamental tasks on graphs where individuals are grouped into clusters or communities based on their graph connectivity. In this work, we aim to examine changes to the community structure of the user-user mentions network around the time of COP events. To this end, we utilize the fast and scalable Louvain algorithm~\cite{blondel2008fast} to detect communities on individual snapshots of the temporal graph. The Louvain algorithm optimizes the \emph{modularity} $Q$ of the graph, defined as follows in a directed graph,
\begin{equation}
    Q = \frac{1}{2m} \sum_{ij} [\mat{A}_{ij} - \frac{k_i k_j}{2m}] \delta(c_i, c_j)
\end{equation}
where $\mat{A}$ is the weighed adjacency matrix of the graph, $k_i$ and $k_j$ are the sum of the weights of edges of nodes $i,j$ respectively, $m$ is the sum of all of the edge weights in the graph, $c_i$ and $c_j$ are the communities of nodes $i,j$ and lastly,  $\delta$ is the kronecker delta function. 

The Louvain algorithm has two phases which are interactively applied. First, all nodes in the graph is assigned its own unique community. Then, the algorithm decides if moving a node from its own community to its neighbors' community improves the modularity score $Q$. The node is then placed into its neighbor's community which sees the most increase in modularity. In the second phase, the algorithm groups all nodes in the same community and builds a new network where nodes are the communities from before. After this creation, the first phase then starts again. The algorithm terminates when no modularity increase can be observed. The complexity of the Louvain algorithm is $O(n \cdot \log n )$ where $n$ is the number of nodes. Note that by design, the Louvain algorithm constructs hierarchical communities as it iteractively groups communities into larger ones. 


\subsection{Sentiment Analysis}
Sentiment analysis is a technique used to determine the emotional tone behind a piece of text, whether \emph{positive}, \emph{negative}, or \emph{neutral}. In the project, the sentiment analysis is used to analyze the overall sentiment of tweets related to climate change. By analyzing the sentiment of social media content, we can understand the emotions associated with different topics related to climate change such as climate policy, environmental disasters or scientific research. Sentiment analysis also helps identify patterns in the emotional tone of different groups, such as climate change supporters or deniers.

\begin{figure}[t]
  \centering
  \includegraphics[width=0.4\textwidth]{figs/sentiment_analysis.png}
  \caption{Distribution of \emph{positive}, \emph{negative} and \emph{neutral} tweets.}
  \label{fig:sentiment_image}
  \vskip -0.2in
\end{figure}

Additionally, sentiment analysis is used to monitor the impact of real-world events on public opinion towards climate change. For example, sentiment analysis can track how the emotional tone of social media posts changes after a natural disaster, political decision, or climate-related news event. Here, we used the \href{https://textblob.readthedocs.io/en/dev/}{TextBlob library} to detect the sentiments of the tweets which determined whether the texts were positive, negative or neutral but did not provide the sentiments as per the supporters favor or denial. Hence, we got this result from TextBlob as depicted by the pie chart in Figure~\ref{fig:sentiment_image}.

\subsection{Topic Modeling}
Topic models are a class of unsupervised machine learning that allows us to extract topics from a large corpus of text data. They are  powerful techniques that are commonly used for identifying patterns and themes in large text datasets. A typical topic model works by identifying groups of words that tend to co-occur in the same documents or tweets. These groups of words are known as "topics" and can provide insights into the underlying themes and issues that are present in the data. Topic modeling is often used in text analysis applications, such as market research, and social media analytics. In our analysis of  opinions on Twitter, we used topic modeling to identify the main topics of conversation related to climate change. By using the mini-batch non-negative matrix factorization (NMF) algorithm \cite{10.1162/NECO_a_00168}, we were able to efficiently extract topics from a large-scale dataset and gain insights into the key themes and issues that are salient to the public.

 The mini-batch NMF algorithm  works by iteratively updating two matrices, $W$ and $H$, that together approximate the original document-word statistic matrix $X\approx HW$. $X$ usually is a term frequency–inverse document frequency (TF-IDF) score matrix describing the weighted frequency of each word  in each document.  The matrix $W$ represents the topic-word matrix, where each row corresponds to a topic and each column corresponds to a word. The matrix $H$ represents the document-topic matrix, where each row corresponds to a document (tweet) and each column corresponds to a topic. During each iteration of the algorithm, a mini-batch of the data is randomly sampled and used to update the values of $W$ and $H$. We chose mini-batch NMF from bunches of topic modeling approaches due to its scalability and fast convergence speed.



==> Preliminary_Work.tex <==
\section{Preliminary Work}

In this section, we describe the current progress and preliminary work that we have achieved in community detection, natural language processing and topic modeling areas. 

\subsection{Community Detection} \label{sub:coms}

\begin{figure}[t]
\centering
\begin{subfigure}{.4\textwidth}
  \centering
  \includegraphics[width=\linewidth]{figs/density.pdf}
  \caption{Density of the graph snapshot}
  \label{Fig:density}
\end{subfigure}%
\begin{subfigure}{.4\textwidth}
  \centering
  %\includegraphics[width=.4\linewidth]{image1}
  \includegraphics[width=\linewidth]{figs/num_clusters_res1.pdf}
  \caption{number of communities} 
  \label{Fig:num_coms}
\end{subfigure}
\caption{
The evolution of a). the graph density and b). number of communities in each graph snapshot of the user-user mentions network constructed from tweets.}
\label{Fig:adv_stats}
\vskip -0.2in
\end{figure}



\begin{figure}[t]
\centering
\begin{subfigure}{.35\textwidth}
  \centering
  \includegraphics[width=\linewidth]{figs/COPs/COP18_clusters.pdf}
  \caption{COP 18}
  \label{Fig:cop18}
\end{subfigure}%
\begin{subfigure}{.35\textwidth}
  \centering
  %\includegraphics[width=.4\linewidth]{image1}
  \includegraphics[width=\linewidth]{figs/COPs/COP19_clusters.pdf}
  \caption{COP 19} 
  \label{Fig:cop19}
\end{subfigure}
\begin{subfigure}{.35\textwidth}
  \centering
  \includegraphics[width=\linewidth]{figs/COPs/COP20_clusters.pdf}
  \caption{COP 20}
  \label{Fig:cop20}
\end{subfigure}%
\begin{subfigure}{.35\textwidth}
  \centering
  %\includegraphics[width=.4\linewidth]{image1}
  \includegraphics[width=\linewidth]{figs/COPs/COP21_clusters.pdf}
  \caption{COP 21} 
  \label{Fig:cop21}
\end{subfigure}
\caption{
The number of communities detected by the Louvain algorithm around a). COP 18, b). COP 19, c). COP 20 and d). COP 21 event.} 
\label{Fig:cop20and21}
\vskip -0.2in
\end{figure}

As a first attempt, we hypothesize that the community structure, particularly the number of communities might vary significantly surround climate change events such as COP. Figure~\ref{Fig:adv_stats} shows the evolution of the graph density over time as well as the number of communities detected by the Louvain algorithm as described in Section~\ref{sub:louvain}. Note that the density of the graph also affects the community structure as dense graphs are likely to have smaller number of communities. Outside of the peak at the beginning of the dataset and the peak around COP 17, the graph remains quite dense. On the other hand, the number of communities seem to increase over time with local peaks periodically. 

Next, we examine the community structure of graph snapshots surround COP events (10 weeks before and 10 weeks after) with the Louvain algorithm. Figure~\ref{Fig:cop20and21} shows the change in number of communities around COP 18 to 21. For COP 18 and 19, there is a decrease in the number of communities. For COP 20 and COP 21, there seem to be an increase of communities. Therefore, it is difficult to directly draw conclusion from these observations. This is also expected as the Louvain algorithm is computed based the graph structure alone and doesn't utilize the tweet text and other edge features. 



\subsection{Natural Langauage Processing}

From the results that we get from the sentiment of the tweets, we understand that its vague to identify the texts as towards climate change or not. Hence, we consider to not move forward with the sentiments analysis of the tweets as the result seems quiet ambiguous.

By combining sentiment analysis with other techniques such as network analysis and topic modeling, we may gain a deeper understanding of the dynamics of climate change communities on social media and how real-world events shape public opinion. This information can be used to develop effective communication strategies, address misinformation campaigns and promote climate change awareness.


\subsection{Topic modeling}
We first tokenized the tweets data and then trained the mini-batch NMF model on the preprocessed corpus by setting the number of topics as 10. We utilized the scikit-learn toolkit to run mini-batch NMF model. The training algorithm was run for iterations until convergence, i.e., a set of stable topics was obtained.  After the matrix factorization had been done, we looked at the topic-word score matrix $W$ and described each topic by the words with the highest relevance score. 
Figure~\ref{Fig:topics} shows three obtained representative topics with their top 20 words about \emph{politics}, \emph{\ch{CO2} emission}, and \emph{weather}. The \emph{politics} topic is related to politicians (e.g., Trump), organizations (e.g., EPA) and actions to address and mitigate climate change. The \emph{\ch{CO2} emission} topic includes global warming, Arctic ice melting, and sea level rising as consequences of \ch{CO2} emission. The \emph{weather} topic shows people's concern about extreme and abnormal weather caused by global warming. 

\begin{figure}[t]
\centering
\vskip 0.12in
\includegraphics[width=0.8\linewidth]{figs/Topics.png}
\caption{Significant topics extracted from the corpus.}
\vskip -0.2in
\label{Fig:topics}
\end{figure}

